NTPP: Generative Speech Language Modeling for Dual-Channel Spoken Dialogue via Next-Token-Pair Prediction

Inspired by the impressive capabilities of GPT-4o, there is growing interest in enabling speech language models (SLMs) to engage in natural, fluid spoken interactions with humans. Recent advancements have led to the development of several SLMs that demonstrate promising results in this area. However, current approaches have yet to fully exploit dual-channel speech data, which inherently captures the structure and dynamics of human conversation. In this work, we systematically explore the use of dual-channel speech data in the context of modern large language models, and introduce a novel generative modeling paradigm, Next-Token-Pair Prediction (NTPP), to enable speaker-independent dual-channel spoken dialogue learning using decoder-only architectures for the first time. We evaluate our approach on standard benchmarks, and empirical results show that our proposed method, NTPP, significantly improves the conversational abilities of SLMs in terms of turn-taking prediction, response coherence, and naturalness. Moreover, compared to existing methods, NTPP achieves substantially lower inference latency, highlighting its practical efficiency for real-time applications.

==> NTPP_v4_arXiv/sections/exp.tex <==
\section{Experiments}

\subsection{Dataset and Baselines}
\textbf{Dataset.}
Our NTPP is trained using a \textit{two-stage pipeline}. In the first stage, we establish the SLM with foundational speech capabilities by training the model on three speech datasets, totaling approximately 140,000 hours. This phase focuses on both speech understanding and synthesis. Unlike other models \cite{fang2024llama,mini-omni} that require additional text alignments, our approach follows a textless learning paradigm. This eliminates the need for speech-text alignment, reducing data preprocessing requirements and significantly increasing the amount of available training data. In the second stage, we equip our SLMs with the ability to listen and speak simultaneously through \method training. For this, we leverage the Fisher dataset \cite{cieri2004fisher}, which contains 2,200 hours of phone conversations between randomly paired participants discussing predefined topics. A key advantage of the Fisher dataset is that each speaker’s audio is recorded on separate channels, providing high-quality dual-channel speech streams essential for \method training. Since the original audio is sampled at 8kHz, we use Librosa \footnote{https://librosa.org/doc.} to upsample it to 16kHz for consistency with our training setup. 

\textbf{Baselines} We evaluate \method's performance by comparing it with established generative speech systems. In terms of turn-taking statistics within generated dialogues, we compared \method specifically with dGSLM \cite{dGSLM}, as it represents a comparable full-duplex generative model trained on the Fisher dataset. Following dGSLM's setting \cite{dGSLM}, we include a cascaded baseline which consists of an Automatic Speech Recognition(ASR) model, followed by a text-based
language model and a Text-To-Speech (TTS) module. 
Following the settings of \cite{dGSLM}, we select wav2vec2-large\cite{Wav2Vec}, KenLM\cite{kenlm}, and Google TTS API as the modules respectively. For assessing the meaningfulness and naturalness of the interaction, we extend our comparison to include Moshi \cite{moshi} and SyncLLM \cite{SyncLLM}. Notably, SyncLLM is a full-duplex dialogue agent designed for real-time, overlapping speech interactions through the joint, streaming processing of speech input and output.






\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/loss_dual_axis.pdf}
    \caption{Comparison of training loss curves across different models. Solid lines show the training progress for different foundation models. Dashed lines represent an ablation study comparing a model trained with textual data (w Text) versus without (w/o Text).}
    \label{fig:loss}
\end{figure}

\begin{table*}[t]
\centering
\caption{Turn-taking statistics (event occurrences and durations/min) for generated dialogues, compared to ground truth using mean absolute differences ($|\Delta|$) between predicted and ground truth values. NTPP model results cover different temperature settings [0.1, 0.5, 0.9]. Lower $|\Delta|$ values indicate better performance, with the best results highlighted in bold.}
\label{tab:linguistic_quality_modified}
\scalebox{0.9}{
\begin{tabular}{ccccccccccc}
\toprule
 \textbf{Model} & \multicolumn{4}{c}{\textbf{Number of occurrences / min}} & \multicolumn{4}{c}{\textbf{Cumulated duration /min}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
   & \textbf{$|\Delta$IPU$|$} & \textbf{$|\Delta$Pause$|$} & \textbf{$|\Delta$Gap$|$} & \textbf{$|\Delta$Overlap$|$} & \textbf{$|\Delta$IPU$|$} & \textbf{$|\Delta$Pause$|$} & \textbf{$|\Delta$Gap$|$} & \textbf{$|\Delta$Overlap$|$} \\
\midrule
 dGSLM w/o CA  & 3.9 & 2.9 & 3.6 & 1. & 12.1 & 8.3 & 1.4 & 2.5 \\
 dGSLM & 1.6 & 3.4 & 2. & 2.9 & 4.6 & 3.6 & 1.8 & 1.9 \\
 LSLM & 2.2 & 3.6 & 2.4 & 3.2 & 4.1 & 3.4 & 1.5 & 2.3 \\
 Cascaded & 4.1 & 7.0 & 7.4 & 6.5 & 4.3 & 5.5 & 0.9 & 3.6 \\
\midrule
 $\method_{0.1}$ & 1.4 & 2.1 & 2.0 & 1. & 3.2 & \textbf{2.5} & 1.2 & 2.1 \\
 $\method_{0.5}$ & 1.5 & \textbf{1.9} & 1.8 & 1.5 & \textbf{2.9} & 3.0 & \textbf{0.9} & 2.2 \\
 $\method_{0.9}$ & \textbf{1.3} & 2.3 & \textbf{1.5} & \textbf{0.9} & 3.3 & 2.8 & 1.4 &  \textbf{1.9} \\
\bottomrule
\end{tabular}}
\label{distribution}
\end{table*}


\vspace{-5pt}

\subsection{SLM Training $\&$ Implementation Details}
\paragraph{Audio Tokenizer \& Token Vocoder.} We train an RVQ speech tokenizer based on \cite{soundstream}, which encodes each second of audio into 40 discrete tokens from a codebook of size 4096. Due to the limitations of the single-speaker token vocoder presented in \cite{NEURIPS2020_c5d73680}, we train a multi-speaker HiFi-GAN to decode speech signals from discrete tokens. The HiFi-GAN architecture consists of a generator and multiple discriminators. The generator uses look-up tables to embed discrete representations and the embedding sequences are up-sampled by a series of blocks composed of transposed convolution and a residual block with dilated layers. The speaker embedding is concatenated to each frame in the up-sampled sequence. The discriminator features a Multi-Period Discriminator and a Multi-Scale Discriminator, which have the same architecture as \cite{NEURIPS2020_c5d73680}. 

\vspace{-10pt}
\paragraph{LLM Backbones.} We leverage three well-known LLMs as the backbone of our SLM: LLaMA 3.1–8B \cite{Llama3}, Mistral-7B-v0.1 \cite{mistral}, and Gemma-2-9B \citep{gemma}. We evaluate the performance of SLMs obtained by training these LLMs with the NTP objective on a large-scale single-channel audio dataset. Perplexity on the test set is used as the evaluation metric. Figure~\ref{fig:loss} shows the training loss curves over time for all three models. Each model demonstrates a consistent downward trend, indicating effective learning. Mistral-7B and Gemma show comparable learning dynamics, while LLaMA 3.1—known for its strong reasoning capabilities in text—achieves lower training loss more quickly. This finding supports our hypothesis that stronger text-based models serve as more effective initializations for continual speech learning, consistent with the perspective of treating audio as a new language. 

Perplexity curves highlights that during the pre-training phase, the \method model demonstrates superior performance when trained exclusively on audio data (``w/o Text") compared to when trained with both audio and its ASR text transcriptions (``w Text"). Specifically, the audio-only approach leads to significantly faster convergence and consistently lower perplexity—a measure indicating better predictive capability of the model. 
The results show that the audio-only setting leads to significantly faster convergence and consistently lower perplexity throughout training. This indicates that eliminating the ASR transcript—which may introduce recognition errors or redundancy—allows the model to focus on more informative acoustic cues, thereby facilitating more stable and efficient learning. In contrast, the inclusion of textual supervision appears to slow optimization and result in higher perplexity, suggesting potential modality interference.

\subsection{Turn-taking Event Distribution}

Following the experimental setting in dGSLM \cite{dGSLM}, we evaluate the dialogue systems with turn-taking capabilities using corpus-level statistics \cite{ardila2019common} and testing on the Fisher dataset \cite{cieri2004fisher}. We evaluate the linguistic quality and turn-taking dynamics of generated dialogues using various models, as shown in Table~\ref{distribution}. The detailed evaluation settings are in the Appendix~\ref{Dialogue linguistic quality}. LSLM \cite{LSLM} integrates speaker channels at the embedding layer and only predicts the speech tokens from the assistant channel, demonstrating a notable reduction in the number of Inter-Pausal Units (IPUs) and gaps, indicating smoother transitions between speakers. The dGSLM \cite{dGSLM}, particularly with the cross-attention module, shows a significant decrease in the cumulative duration of pauses and gaps, suggesting more fluid and continuous dialogue. Comparatively, \method exhibits balanced performance with moderate reductions in both the number and duration of turn-taking events, highlighting their potential for generating natural and coherent dialogues. These findings underscore the importance of model architecture in optimizing dialogue flow.




\subsection{Interruptions \& Reflective Pause}

We further develop a comprehensive evaluation framework comprising 400 diverse conversational scenarios specifically designed to systematically capture natural dialogue dynamics, with an emphasis on pauses and interruptions. These scenarios are carefully crafted using GPT-4 to reflect the complexity and nuance of human interactions. We then use ChatTTS\cite{chattts} to synthesize high-quality speech from the generated text, effectively mimicking the acoustic characteristics of real-world conversations. As shown in Figure~\ref{interaction_accuracy}, \method demonstrates closer alignment with human reference judgments, which are meticulously established through manual annotation by human evaluators, in both speaking-up and interruption scenarios when acting as a listener. For instance, informing its response strategy, \method employs Voice Activity Detection (VAD) and considers a silence state to have been reached after 200ms of continuous non-speech is detected, facilitating its decisions on when to speak or acknowledge a pause. This suggests that \method more effectively captures the subtleties of human conversational behavior compared to other models. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/Combined_Interruptions_Reflective_Pause.pdf}
    \caption{NTPP, when acting as a listener, shows closer alignment with Human Reference judgments in both speaking up and interrupting scenarios.}
    \label{interaction_accuracy}
\end{figure}

\begin{table*}[h]
\centering
\caption{Human evaluation results across different SLMs. Meaningfulness (Meaning.) and Naturalness (Nat.) scores (ranging from 1 to 5) represent mean estimates and their standard errors (shown in parentheses), reported both overall and separately for the Fisher and CANDOR datasets.}
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Overall}} & \multicolumn{2}{c}{\textbf{Fisher}} & \multicolumn{2}{c}{\textbf{CANDOR}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
 & \textbf{Meaning. $\uparrow$} & \textbf{Nat. $\uparrow$} & \textbf{Meaning. $\uparrow$} & \textbf{Nat. $\uparrow$} & \textbf{Meaning. $\uparrow$} & \textbf{Nat. $\uparrow$} \\
\midrule
dGSLM & 1.38 (0.10) & 3.85 (0.12) & 1.82 (0.09) & 4.10 (0.13) & 1.51 (0.12) & 2.85 (0.18) \\
SyncLLM & 3.85 (0.06) & 4.10 (0.05) & 4.10 (0.04) & 4.33 (0.08) & 3.85 (0.09) & 3.91 (0.08) \\
Moshi & 3.90 (0.07) & 3.95 (0.06) & 3.20 (0.10) & 3.90 (0.08) & 3.95 (0.08) & 3.95 (0.08) \\
\textbf{\method} & \textbf{3.95 (0.04)} & \textbf{4.15 (0.06)} & \textbf{4.10 (0.06)} & \textbf{4.42 (0.06)} & \textbf{4.05 (0.04)} & \textbf{4.05 (0.10)} \\
GT & 4.90 (0.01) & 4.95 (0.02) & 4.90 (0.03) & 4.90 (0.04) & 4.90 (0.02) & 4.95 (0.02) \\
\bottomrule
\end{tabular}
\label{human_evaluation}
\end{table*}



\begin{table*}[t]
\centering
\caption{Linguistic quality and turn-taking metrics under speaker-swapped inference. Reported values denote the absolute difference between deviation metrics $\Delta M$ (e.g., $\Delta \text{IPU}$) under the original and swapped speaker orders, computed as $|\Delta M_{\text{original}} - \Delta M_{\text{swapped}}|$. Lower values indicate higher robustness to speaker order permutation. 
}
\label{tab:linguistic_quality_speaker_independent}
\scalebox{0.9}{\begin{tabular}{lc cccc cccc}
\toprule
\textbf{Split} & \textbf{Model} & \multicolumn{4}{c}{\textbf{Number of Occurrences / min}} & \multicolumn{4}{c}{\textbf{Cumulated Duration / min}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & \textbf{$|\Delta$IPU$|$} & \textbf{$|\Delta$Pause$|$} & \textbf{$|\Delta$Gap$|$} & \textbf{$|\Delta$Overlap$|$} & \textbf{$|\Delta$IPU$|$} & \textbf{$|\Delta$Pause$|$} & \textbf{$|\Delta$Gap$|$} & \textbf{$|\Delta$Overlap$|$} \\
\midrule
\multirow{3}{*}{\textbf{Train}} 
& dGSLM   & 0.05 & 0.14 & \textbf{0.04} & 0.06  & 0.09 & \textbf{0.15} & \textbf{0.11} & 0.09  \\
& Moshi   & 0.43 & 0.32 & 0.29 & 0.29  & 0.30 & 0.56 & 0.55 & 0.58  \\
& $\method$ & \textbf{0.03} & \textbf{0.07} & 0.07 & \textbf{0.05} & \textbf{0.06} & 0.18 & 0.14 & \textbf{0.06} \\
\midrule
\multirow{3}{*}{\textbf{Test}} 
& dGSLM   & 0.20 & 0.15 & \textbf{0.18} & 0.21  & 0.39 & \textbf{0.32} & \textbf{0.41} & 0.32  \\
& Moshi   & 0.43 & 0.38 & 0.37 & 0.39  & 0.57 & 0.62 & 0.84 & 0.68  \\
& $\method$ & \textbf{0.18} & \textbf{0.14} & 0.19 & \textbf{0.20} & \textbf{0.35} & 0.38 & 0.45 & \textbf{0.24} \\
\bottomrule
\end{tabular}}
\label{tab:speaker-independent}
\end{table*}

\subsection{Human Evaluation}
We follow the evaluation protocol from~\cite{beyond} and conduct a human study involving 25 annotators with native-level English proficiency. Adopting the Mean Opinion Score (MOS) framework, we use a 5-point Likert scale to evaluate the Naturalness (N-MOS) of turn-taking and the Meaningfulness (M-MOS) of the generated dialogue content. Table~\ref{human_evaluation} presents a comparison of \method with various baselines in terms of both naturalness and meaningfulness. We also include performance comparisons on the out-of-distribution Candor test set~\cite{candor} to assess generalization.

\subsection{Inference Latency}
In multi-turn interactions, latency is a crucial metric for assessing the performance of speech interaction models, as it captures the time between receiving the end of input speech and the start of output speech, directly impacting user experience. As shown in Figure~\ref{fig:latency}, our \method consistently achieves lower inference latency than Moshi, especially as the number of turn-taking rounds increases. We attribute this advantage to \method's efficient memory usage: it maintains a single KV Cache, while Moshi requires two separate KV Caches for the two separate transformers. This difference becomes increasingly significant as conversational context grows longer. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/latency_comparison_with_noise.pdf}
    \caption{Our method (blue) demonstrates lower latency growth compared to Moshi's linear degradation(red), maintaining response times below perceptual thresholds (220 ms) across all rounds.}
    \label{fig:latency}
\end{figure}

\subsection{Speaker Independence}
To assess the speaker-independence of various models, we conduct a speaker-swapped evaluation. All models are first trained on the dual-channel Fisher dataset \cite{cieri2004fisher} using the canonical speaker order. We reverse the input speaker sequence without any additional fine-tuning or adaptation. This setup allows us to test whether a model's performance remains stable when the roles of the two speakers are exchanged—an essential indicator of robustness and generalization in dialogue turn-taking modeling. We evaluate this on \textit{both the training and test sets}. As shown in Table~\ref{tab:linguistic_quality_speaker_independent}, both dGSLM and \method exhibit minimal variation in key turn-taking metrics under speaker-swapped conditions—nearly zero variation on the training set and consistently low variation on the test set—demonstrating strong speaker-independent behavior. Moshi shows substantial deviations in metrics such as the number and duration of IPUs, pauses, gaps, and overlaps. These findings suggest that Moshi relies on speaker-conditioned generation (due to its modeling of conditional distributions), resulting in degraded performance when the input speaker order is reversed.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.97\linewidth]{figures/combined_figure.pdf}
    \caption{Comparative performance analysis. (a) Ablation study of NTPP model training stages, illustrating perplexity versus training steps for the full two-stage model and variants lacking either stage one or stage two. For better visualization, we trim the stage one training steps to be the same as stage two. (b) Comparison of VQ and RVQ model training loss as a function of training steps.} 
    \label{fig:ablation_phase}
\end{figure}

\vspace{-5pt}
\subsection{Ablation Studies}
We further investigate the importance of two-stage training and the use of an RVQ tokenizer in this section. As shown in Figure~\ref{fig:ablation_phase} (a), our two-stage training strategy consistently achieves lower perplexity compared to the one-stage approach, which omits pretraining on single-channel audio. This suggests that pretraining on single-channel audio provides a strong foundation, significantly improving performance on subsequent dual-channel speech learning. As expected, omitting the second-stage NTPP training on dual-channel speech also leads to performance degradation. Figure~\ref{fig:ablation_phase} (b) compares training loss between VQ and RVQ tokenizers, with RVQ yielding consistently lower loss, highlighting the importance of developing extended solutions tailored to this tokenizer. 







